Sample Complexity for Quadratic Bandits: Hessian Dependent Bounds and Optimal Algorithms

In stochastic zeroth-order optimization, a problem of practical relevance is understanding how to fully exploit the local geometry of the underlying objective function. We consider a fundamental setting in which the objective function is quadratic, and provide the first tight characterization of the optimal Hessian-dependent sample complexity. Our contribution is twofold. First, from an information-theoretic point of view, we prove tight lower bounds on Hessian-dependent complexities by introducing a concept called energy allocation, which captures the interaction between the searching algorithm and the geometry of objective functions. A matching upper bound is obtained by solving the optimal energy spectrum. Then, algorithmically, we show the existence of a Hessian-independent algorithm that universally achieves the asymptotic optimal sample complexities for all Hessian instances. The optimal sample complexities achieved by our algorithm remain valid for heavy-tailed noise distributions, which are enabled by a truncation method.

==> KL.tex <==
%todo: lower to app
\subsection{A Gentle Example: 
The 1D Algorithm}\label{sec:alg1d}

The proposed algorithm operates alternatively in two phases, a global search phase and a local search phase. We presented an illustration using the $d=1$ case, where the optimal complexity can be achieved using a simpler routine. 
\begin{prop}
For $d=1$ and sufficiently small $\delta$, there is an algorithm that achieves an error of $f(x_T)-f^* \leq\epsilon$ w.p. $1-\delta$ with a sample complexity of $\tilde{O}\left(\epsilon^{-\frac{2\alpha+5}{3}}\log(1/\delta)\right)$.
\end{prop}
\begin{proof}
 As 
%for the 1D case
 described in Algorithm 1, the proposed routine maintains a variable $x_{\textup{c}}$ over $T$ iterations.
  We ensure that the gap between $f(x_{\textup{c}})$ and  $f^*$  is upper bounded by a quantity $g$ with high probability, so that if $g$ is reduced by a constant factor each iteration, then the stated learning error $\epsilon$ can be achieved within  logarithmic number of iterations.   %within each iteration by a constant factor 

\begin{algorithm}
\caption{1D Search}\label{alg:cap}
\begin{algorithmic}
\State Initialize ${x}_{\textup{c}}=0$, $g=\left(\frac{4C_2}{C_1^2} \right)^{\frac{1}{2\alpha-1}}$. 
%\While {$g\geq \epsilon$} 
%\State 
Let $T= \left\lceil 2{\log_{2} (g/\epsilon)}\right\rceil$. 

\For{$t\leftarrow  1 $ to $T$}
%\State Let $\delta_t=\frac{\delta}{2\cdot 2^{T-t}}$.


\State Global Search Phase:
%\State Initialize  $L=\frac{2^{1+\alpha} g^{1-\alpha}}{C_1(1-\alpha)}$.  
% Let  $C_0=\frac{g}{L} $.  

\State Let $C_0= \frac{1}{2}{{C_1(1-\alpha)}{(g_t/2)^{\alpha}}}$, $L_{\textup{th}}= \left(\frac{1}{C_0^2}\sqrt{\frac{g^5}{C_2}}\right)^{\frac{1}{3}}$, $\delta_t=\frac{\delta}{ 2^{T-t}} $. Initialize $L=\frac{g}{C_0}$.

%Let %\in[\frac{5C_0}{C_3}, 3C_0]$
\While{$L> L_{\textup{th}}$} %{$t_2\leftarrow  1 $ to $ T_2$}

\State Let  $\Delta_C=C_0\left({L_{\textup{th}}}/{2L}\right )^{\frac{2}{3}}$,  $\epsilon_L=\frac{1}{8}{\Delta_C\cdot L}  $, $\delta_{L}=\delta_t \cdot \frac{L_{\textup{th}}}{24L}$, $\mathcal{S}=\{x_{\textup{c}}-\frac{L}{2},x_{\textup{c}}, x_{\textup{c}}+\frac{L}{2}\}$

\State Let  $x_{\textup{c}}=\textup{argmin}_{y\in\mathcal{S}} (C_0+\Delta_C)\cdot |y-x_{\textup{c}}|+$Sample$\left(y,\epsilon_L,\delta_{L}\right)$,  $L=\frac{1}{2}L$. 
\EndWhile

%\State $\boldsymbol{x}=$Uniform search$(\mathcal{B}, \boldsymbol{x}, \frac{g}{3}, \frac{\delta}{2T_1})$,  $g=(\frac{2}{3})^{\alpha} g$
 %other half)$


\State Local Search Phase: 
\State Let $N=2\left\lceil L /\sqrt{\frac{g}{C_2}} %{C_2}^{\frac{1}{2}} g^{-\frac{2\alpha-1}{3}}
\right\rceil$, $\epsilon_{\textup{s}}=\frac{g}{16}$, $\delta_{\textup{s}}=\delta_t\cdot\frac{1}{2(N+1)}$,  $\mathcal{D}=\{x_{\textup{c}}-L, x_{\textup{c}}-L+\frac{2L}{N},..., x_{\textup{c}}+L\}$


\State Let $x_{\textup{c}}=\textup{argmin}_{{y}\in\mathcal{D}}$ Sample$\left({y},{\epsilon_{\textup{s}}},\delta_{\textup{s}} \right)-2\epsilon_{\textup{s}}\cdot \mathbbm{1}({y}={x}_{\textup{c}})$
\State Let $g=\frac{g}{2}$
\EndFor


\Return $x_c$


~

\Procedure{Sample}{$\boldsymbol{x},\epsilon_{\textup{s}},\delta_{\textup{s}}$}

\Return the average of $\lceil2\epsilon_{\textup{s}}^{-2}\ln\frac{1}{\delta_{\textup{s}}}\rceil$ samples of $f$ at $\boldsymbol{x}=x_n$.
%\State Sample $f$ at $\boldsymbol{x}$ for ${O}(\epsilon_{\textup{s}}^{-2}\ln\frac{1}{\delta_{\textup{s}}})$ times, then assign their average to $y_n$
\EndProcedure
\end{algorithmic}
\end{algorithm}

Each iteration %, the reduction
starts with a  global search phase, where the algorithm maintains an interval $[x_{\textup{c}}-L,x_{\textup{c}}+L]$, of which the length is to be reduced by a factor of $\frac{1}{2}$  through each search step.
The main idea of the algorithm is to ensure that the minimum of $f$ within the interval approximates $f^*$ with high probability, so that %it always suffices to sample within the interval. 
once $L$ is small enough, one can switch to a local search phase, and the approximated minima can be found using a grid search. 
The transition threshold $L_{\textup{th}}$ %(specified by the condition $L>g^{\frac{5-4\alpha}{6}}$)
 is selected to minimize the overall sampling cost (see the analysis at the end of the proof). 

The design and the choice of parameter values in the algorithm are based on the following building blocks. First, 
a subroutine \emph{Sample} is to be used throughout this work, which repetitively samples $f$ at the same point to provide an accurate estimation. Formally, we have the following guarantee, which directly follows from the Hoeffding inequality of sub-Gaussian random variables. % tail bounds of the Gaussian CDF.
\begin{prop}\label{prop:sample}
The Sample function returns a value that is within $(f(\boldsymbol{x})-\epsilon_{\textup{s}},f(\boldsymbol{x})+\epsilon_{\textup{s}})$ w.p. $1-\delta_{\textup{s}}$. 
\end{prop}
We shall always consider the high-probability regime where all sampled results fall into the intervals $(f(\boldsymbol{x})-\epsilon_{\textup{s}},f(\boldsymbol{x})+\epsilon_{\textup{s}})$. The overall error probability is controlled by the union bound.

Besides, we use the following property to set the initialization of $g$, so that we have % by showing that if 
$f(x_{\textup{c}})-f^*\leq g$ at the beginning of the first iteration.  The proof of Proposition \ref{prop:ele} can be found in appendix \ref{app:ppele}. 
\begin{prop}[Boundedness]\label{prop:ele}
For any differentiable function $f$ that satisfies smoothness and KL inequality for all   $\boldsymbol{x}\in\mathcal{X}$, i.e., $f(\boldsymbol{x})\leq f(\boldsymbol{0})$, we have 
\begin{align*}f(\boldsymbol{0})-f^*\leq\left(\frac{4C_2}{C_1^2} \right)^{\frac{1}{2\alpha-1}}.
\end{align*}
Moreover, for any $\boldsymbol{x}\in\mathcal{X}$ there is a global minimum of $f$ within an $L_2$-distance of $L_{\boldsymbol{x}}\triangleq \frac{(f(\boldsymbol{x})-f^*)^{1-\alpha}}{C_1(1-\alpha)}$. For any $\boldsymbol{x}\in\mathcal{X}$ and $L\leq L_{\boldsymbol{x}}$, let $\mathcal{B}$ be the $L_2$-ball centered at $\boldsymbol{x}$ with a radius of $L$.  If %$f(\boldsymbol{y})> f^*+(C_1(1-\alpha)(L_{\boldsymbol{x}}-L))^{\frac{1}{1-\alpha}} $
$L_{\boldsymbol{y}}>L_{\boldsymbol{x}}-L$ for all $\boldsymbol{y}\in\partial{B}$, then there is a global minimum of $f$ 
within $\mathcal{B}$. %on the surface of $\mathcal{B}$.
%$\mathcal{B}\triangleq \left\{\boldsymbol{y}\in \mathbb{R}^d\ \Big{|}\ ||\boldsymbol{y}-\boldsymbol{x}||_2\leq 
%an $L_2$-distance of $\frac{|f(\boldsymbol{x})-f^*|^{1-\alpha}}{C_1(1-\alpha)}$ to $\boldsymbol{x}$ if . %, a global minimum of $f$ exists within $\mathcal{B}$.
\end{prop} 


%  and the interval length $L$.  Its proof can be found in
Given these facts, our algorithm is designed to ensure that for any fixed iteration, if $f(x_{\textup{c}})-f^*\leq g$  holds at the beginning, the same inequality holds with high probability at the end.
%We prove the algorithm achieves the stated  guarantees through an inductive approach. %
%First, the initialization of $g$ is configured based on 
 To avoid confusion, we denote the value of $g$ at the beginning of the iteration by $g_{t}$, so at the end of of the iteration we have $f(x_{\textup{c}})-f^*\leq {g_t}/2$.  %, and the $g$ value at the end by $g_{t+1}$.
 
%Recall that $g_t$ is reduced by half after each iteration. 

The gist of the global search phase is to %maintain the interval $[x_\textup{c}-L,x_\textup{c}+L]$ such 
ensure that throughout the entire process, either we have $f(x_{\textup{c}})-f^*\leq {g_t}/2$, or a global minimum of $f$ exists in $(x_\textup{c}-L,x_\textup{c}+L)$. 
By the second and third statement of Proposition \ref{prop:ele}, this condition can be implied if $\boldsymbol{x_{\textup{c}}}\in\mathcal{X}$ and both %that the interval 
$f(x_{\textup{c}}-L)$ and $f(x_{\textup{c}}+L)$ are greater than $f(x_{\textup{c}})-2C_0\cdot L$. %This is how the parameter $C_0$ is chosen. However,
In the ideal case where the function value of $f$ can be exactly obtained, one can apply a binary search to maintain the above property while decreasing the interval length $L$. However, due the stochastic nature of the optimization problem, we need to consider an alternative list of gradually relaxed constraints to reduce the sample complexity.  Hence, we instead ensure the following stronger condition to hold %(with high probability)
 at the end of each search step (i.e., each inner iteration). %\footnote{This inequality is designed to control the overall sample complexity. } %Relevant details are provided at the end of the proof. }
\begin{align}\label{ineq:1ds2}
   f(x_{\textup{c}}\pm L)\geq  f(x_{\textup{c}})-\left(C_0+\Delta_C\right) L.
\end{align}
%where $\Delta_C\triangleq C_0 \left(L_{\textup{th}}/{2L}\right )^{\frac{2}{3}}$.  
As shown in the detailed analysis in Appendix \ref{app:pkl1dd}, the presented global search guarantees the above condition, with the number of samples required   for each search step being inversely proportional to the square of the increment of $\Delta_C$ times $L$. Therefore, we design the relaxation parameter $\Delta_C$ to be exponentially dependent on the number of inner  iterations to compensate the exponential decay of $L$, to minimize the overall sample complexity. 
 
 %We use induction to prove that The relevant details are presented in 



Note that in both global search and local search phases,  $x_{\textup{c}}$ is only updated when $f(x_{\textup{c}})$ is known to be decreased with high probability. Hence, we have $x_{\textup{c}}\in\mathcal{X}$ throughout the entire process, which ensures the correctly of the global search algorithm. % and $f(x_{\textup{c}})-f^*\leq g_{t}$ throughout each iteration. % with high probability. 
%For the same reason, given that $g$ is reduces by a factor of $\frac{1}{2}$ within each iteration, we can focus on cases where the initial condition satisfies $f(x_{\textup{c}})-f^*> \frac{1}{2}g$. 

%with high probability at the end of $t$-th iteration..
   %Boundedness: $f(\boldsymbol{0})-f(\boldsymbol{x})<C_1$.
%todo: revise prop, explain guarantee

%First, consider the global search phase, we prove that at the end, where $C_0\triangleq \frac{{C_1(1-\alpha)}{(g_t/2)^{\alpha}}}{2}$. By the second and third statement of Proposition \ref{prop:ele}, this condition ensures that either 



%note that the search algorithm only updates $x_{\textup{c}}$ when $f(x_{\textup{c}})$ is known to decrease with high probability. It remains to consider the case where $x_{\textup{c}}>g_t/2$. According to the earlier conclusion, there is $x^*\in{(x_\textup{c}-L,x_\textup{c}+L)}$ such that $f(x^*)=f^*$. 
%For brevity, let $f^*_{\textup{local}}$ denote the infimum of $f$ within $[x_\textup{c}-L,x_\textup{c}+L]$. Further,

Now we consider the local search phase. Because $f(x_{\textup{c}})$ is non-increasing with high probability. It remains to focus on the case where $x_{\textup{c}}>g_t/2$. According to the earlier conclusion, a global minimum exists within ${(x_\textup{c}-L,x_\textup{c}+L)}$.  
 From the smoothness condition,  any point within a distance of $O\left(\sqrt{\frac{g_t}{C_2}}\right)$ to this global minimum has  a function value no greater than $f^*+O(g_t)$.  Based on this observation, we perform the grid search by letting adjacent sample points having the same distance, i.e.,  setting %choose
  the number of sample points
  $N$ to be $\Theta\left(\left\lceil L_{\textup{th}} /\sqrt{\frac{g}{C_2}}\right\rceil \right)$. 
%evenly partition the interval  ${(x_\textup{c}-L,x_\textup{c}+L)}$ into $N$ segments, so that the distances between the $N$
%search choose the number 
Formally, let $\mathcal{D}$  denote the set of all $N+1$ sample points in the local search and $f^*_{\textup{disc}}$ denote the minimum of $f$ within this discrete set. The smoothness property at $x^*$ implies the following quantization error bound. 
\begin{align*} f^*_{\textup{disc}}-f^*\leq  {C_2}\left(\frac{L}{N}\right)^2\leq\frac{g_t}{4}.
\end{align*}
Therefore, by Proposition \ref{prop:sample}, $x_{\textup{c}}$ is updated to a different point with high probability due to $f(x_{\textup{c}})- f^*_{\textup{disc}}>4\epsilon_{\textup{s}}$, and the updated function value is upper bounded by $f^*_{\textup{disc}}+2\epsilon_{\textup{s}}< f^*+\frac{g_t}{2}$.   

%Again, recall that 
%note that the search algorithm only updates $x_{\textup{c}}$ when $f(x_{\textup{c}})$ is known to decrease with high probability. It remains to consider the case where $x_{\textup{c}}>g_t/2$. According to the earlier conclusion, there is $x^*\in{(x_\textup{c}-L,x_\textup{c}+L)}$ such that $f(x^*)=f^*$. 
%For brevity, let $f^*_{\textup{local}}$ denote the infimum of $f$ within $[x_\textup{c}-L,x_\textup{c}+L]$. Further,

~

As mentioned earlier, the overall error probability can be controlled by the union bound. For each iteration $t$, any global search step calls the sample function three times, incurring an error probability of at most $3\delta_L=\delta_t \cdot \frac{L_{\textup{th}}}{8L}$. Recall that $L$ decays exponentially and is lower bounded by $\frac{1}{2}L_{\textup{th}}$. The total error probability due to global search within this iteration is at most $\frac{1}{2}\delta_t $. Then for the local search, the sample function is called $N+1$ times, and the overall error probability is bounded by $(N+1)\delta_{\textup{s}}=\frac{1}{2}\delta_t$ as well.  Taking all iterations into account, the algorithm returns an ${x}_{\textup{c}}$ with $f({x}_{\textup{c}})-f^*\leq {\epsilon}$ with an error probability of at most $\sum_{t=1}^{T}\delta_t<\delta$.


%Then by union bound and Proposition \ref{prop:sample},  with a probability of at least $1-\frac{\epsilon}{2}$.
%Combine all above results, we have
%$f(\hat{\boldsymbol{x}})-f^*\leq \epsilon$ w.p. $1-\delta$.
%We show that the returned estimator approximates $f^*_{\textup{local}}$ with an error of at most $\frac{3}{4}\epsilon$ with high probability. %with error probability no greater that $\frac{1}{2}\delta$. 
%algorithm updates the interval by comparing $f_1$ and $f_2$. We first consider the case where $f_1\geq f_2$.

%todo: verify x decrease

The sample complexity bound can be analyzed similarly. % as follows. % the costs due to the Sample function. % the sample complexity. 
Consider any iteration $t$. The sampling cost of any global search step is at most $O(\epsilon_L^{-2}\log(1/\delta_L))$, and the total cost within the iteration is at most
 %  , recall that $L$ decays exponentially. The sampling cost is simply bounded by 
 %\begin{align*}
 $O\left(C_0^{-2}L_{\textup{th}}^{-2}\log\left(\frac{1}{\delta_t}\right)\right)={O}\left(g_t^{-\frac{2\alpha+5}{3}}\log\left(\frac{1}{\delta_t}\right)\right)$
%\end{align*}
 for sufficiently small $\delta$. 
Then for the local search, the same Sample function is called $O(N)$ times, each requiring $O(\epsilon_{\textup{s}}^{-2}\log(1/\delta_{\textup{s}}))$ samples. Hence, the total sampling cost for local search is upper bounded by
%\begin{align*}
$O\left(N g_t^{-2}\log\left(\frac{1}{g_t\delta_t}\right)\right)=\tilde{O}\left(g_t^{-\frac{2\alpha+5}{3}}\log\left(\frac{1}{\delta_t}\right)\right).$
%\end{align*}
Using the fact that $g_t$ exponentially depends on $t$,  the overall sample complexity is bounded by  
%To conclude, the proposed algorithm achieves the stated learning performance with a sample complexity of
$\tilde{O}(\epsilon^{-\frac{2\alpha+5}{3}}\log(1/\delta))$.%overall complexity matches the ones stated in theorems.
\end{proof}




\subsection{Dominant Point and Iterative Reduction}
%\subsection{The General Search Algorithm: }
\label{sec:genalg}

To present the general search algorithm, we first state some useful concepts and procedures. For brevity, we shall reuse the Sample function defined in Algorithm \ref{alg:cap}. We will also use Proposition \ref{prop:sample} and Proposition \ref{prop:ele}, which hold for any $d$. % and useful subroutines. 


\begin{defn}[Dominant Point]
Given any set $\mathcal{B}$, function $f$, and fixed $C>0$, we say $\boldsymbol{x}\in \mathcal{B}$ is a \emph{dominant point} of $\mathcal{B}$ if for any $\boldsymbol{y}\in\partial\mathcal{B}$ we have
\begin{align*}f(\boldsymbol{x})< f(\boldsymbol{y})+C||\boldsymbol{y}-\boldsymbol{x}||_2.
\end{align*}
\end{defn}
We prove the following property (see Appendix \ref{app:pp2}), which ensures that any dominant point $\boldsymbol{x}$   on a set $\mathcal{B}$ imposes guarantees  on either the location of a global minimum of $f$, or the  %corresponding
 function value of $\boldsymbol{x}$. 
 \begin{prop}\label{prop:dom_key}%smooth needed for gf
 For any given $f\in\mathcal{F}$ and $C>0$, if $\boldsymbol{x}\in\mathcal{X}$ is a dominant point of a closed set $\mathcal{B}$,  %with some  and $f\in\mathcal{F}$, %and KL inequality holds  within $\mathcal{B}$, 
 then either a global minimum of $f$ can be found within $\mathcal{B}$,
 or  $f(\boldsymbol{x})-f^*\leq \left({    \frac{C}{ C_1(1-\alpha)}}\right)^{\frac{1}{\alpha}}$. %Consider any $C$ satisfying  $$asd$$
 % can choose $C_0$ to match this upper bound
 \end{prop}
%The gist of the proof for the main theorem is that 
A key building block of the proposed algorithm is a function that runs iteratively and each time returns a dominant point from a smaller set (see Algorithm \ref{alg:doms}). More specifically, given any hypercuboid $\mathcal{B}$ and a dominant point $\boldsymbol{x}$, they returns a dominant point  for a smaller hypercuboid, where the length of the longest edge is reduced by at least a factor of $4/5$. %, 
%Each call of the Reduce function increments the parameter $C$ by $2\Delta$ to achieve the needed reduction under noisy observations. 
%The reduction 
%need delta shift
\begin{algorithm}
\caption{}\label{alg:doms}
\begin{algorithmic}
%applies to any reasonable shape?
%\Procedure{KL covering}{$\mathcal{S}$, $C$,  $r$, $\boldsymbol{x}$}
%\State Let $\mathcal{Y}=\varnothing$
%\Do 
%\State Let $\mathcal{Y}$ be a KL-covering parameterized with  $(C_2,r)$ with minimum 
%\State Estimate $f(\boldsymbol{x})$ with x samples
\Procedure{Reduce}{$\mathcal{B}=\prod_{j=1}^d[a_j,b_j]$, %$f$,
 $\boldsymbol{x}=(x_1,...,x_d)$, $C_0$, $\Delta$, %$\epsilon_{\textup{s}}$,
 $\delta_{\textup{r}}$}
\State Let $k=\textup{argmax}_j(b_j-a_j) $, $\epsilon_\textup{r}=\Delta(b_k-a_k)/20$, $(p,q)=$ Balanced Partition$(a_k,b_k,x_k)$,\\
\ \ \ \ \ \ \ \ \ \ $\mathcal{S}_p=\{\boldsymbol{y}=(y_1,...,y_d)\in\mathcal{B}\ |\ y_k=p\}$, $\mathcal{S}_q=\{\boldsymbol{y}=(y_1,...,y_d)\in\mathcal{B}\ |\ y_k=q\}$
\State Let $\mathcal{S}_{\textup{net},p}$, $\mathcal{S}_{\textup{net},q}$ be  $\sqrt{\epsilon_{\textup{r}}/C_2}$-nets of $\mathcal{S}_p$ and $\mathcal{S}_q$, respectively, and $\mathcal{S}=\mathcal{S}_{\textup{net},p}\cup\mathcal{S}_{\textup{net},q}\cup \{\boldsymbol{x}\}$\\
\ \ \ \ \ \ \ \ \ \ $\boldsymbol{y}^*=\textup{argmin}_{\boldsymbol{y}\in\mathcal{S}} (C_0+\Delta)||\boldsymbol{y}-\boldsymbol{x}||_2+$ Sample$(\boldsymbol{y}, \epsilon_\textup{r}, \frac{\delta_{\textup{r}}}{|\mathcal{S}|})$
%\For {$\boldsymbol{y}\in \mathcal{S}_{\textup{net}}$}
%\State Let $\boldsymbol{x}=\boldsymbol{y}^*$, $D=D+3\Delta$, $C=\frac{\Delta }{\max\{C_3,1\}}$
%\State $\hat{f}_{\boldsymbol{y}}$=Sample$(\boldsymbol{y}, \epsilon_\textup{r}, \frac{\delta_{\textup{r}}}{|\mathcal{S}_{\textup{net}}|})$ 
%Estimate $f(\boldsymbol{x})$ with $\tilde{\Theta}((Cr)^{-2})$ samples, and let the result be $\hat{f}_{\boldsymbol{x}}$.
%\State Let  $ F_{\boldsymbol{y}}= \hat{f}_{\boldsymbol{y}}+ D||\boldsymbol{y}-\boldsymbol{x}||_2$ and  $\boldsymbol{y}^*=\textup{argmin}_{\boldsymbol{y}\in\mathcal{Y}}\  F_{\boldsymbol{y}}$
%\EndFor
\If {$\boldsymbol{y}^*\notin \mathcal{S}_p$}
\State $a_k=p$
\EndIf
\If {$\boldsymbol{y}^*\notin \mathcal{S}_q$}
\State $b_k=q$
\EndIf

\Return $(\mathcal{B}^*=\prod_{j=1}^d[a_j,b_j], \boldsymbol{y}^*)$. 
\EndProcedure

~

\Procedure{Balanced Partition}{$a,b,x$}
\ 

\Return $(p,q)=\begin{cases}
(\frac{2x+b}{3}, \frac{x+2b}{3}) & \textup{if }x\in[a,\frac{3a+2b}{5})\\
(\frac{a+x}{2}, \frac{x+b}{2}) & \textup{if }x\in[\frac{3a+2b}{5}, \frac{2a+3b}{5})\\
(\frac{2a+x}{3}, \frac{a+2x}{3})  &\textup{if }x\in[\frac{2a+3b}{5},b]
\end{cases}
$
\EndProcedure

\end{algorithmic}
\end{algorithm}


Formally, we have the following guarantees on the reduce function, which is proved in Appendix \ref{app:pp5}.
\begin{prop}\label{prop:redu}%todo:check: no kl?
For any input $\boldsymbol{x}\in\mathcal{X}$ being a 
 dominant point of the input hypercuboid $\mathcal{B}$ with parameter $C=C_0$, if %$\sqrt{\epsilon_{\textup{r}}}\leq (b_k-a_k)$,
 $f$ satisfies the smoothness condition on $\mathcal{B}\cap \mathcal{X}$ and $C_0+2\Delta\leq\frac{2}{5}C_2(b_k-a_k)$, then w.p. $1-\delta_{\textup{r}}$, the Reduce function returns a pair such that $\boldsymbol{y}^*$ is a dominant point of $\mathcal{B}^*$ with parameter $C=C_0+2\Delta$. Moreover, if $\frac{b_j-a_j}{b_k-a_k}=\Theta(1)$ for each $j\in[d]$ and $\Delta=O(b_k-a_k)=O(1)$, then for any sufficiently small $\delta$, the overall sample complexity is ${O}\left(\frac{ (b_k-a_k)^{\frac{d-5}{2}}}{\Delta^{\frac{d+3}{2}}}\log(\frac{b_k-a_k}{\Delta\delta})\right)$. 
\end{prop}
\subsection{Proof of Achievability Theorems}\label{sec:algpt}

Similar to the 1D case, an expected simple regret of $O(\epsilon)$ is guaranteed once it can be achieved with high probability, i.e., with $\delta= O(\epsilon)$. Therefore, we focus on the algorithm needed for Theorem \ref{thm:2p}, which is presented as Algorithm \ref{alg3}. 
\begin{algorithm}
\caption{General Search Algorithm}\label{alg3}
\begin{algorithmic}
\Procedure{KL Search}{$\epsilon$, $\delta$} %, $\Delta$}
%\State Let $\boldsymbol{y}^*=\boldsymbol{x}_0$
\State Initialize $\boldsymbol{x}=\boldsymbol{0}$, $g=\left(\frac{4C_2}{C_1^2} \right)^{\frac{1}{2\alpha-1}}$.
%\While {$g\geq \epsilon$} 
 Let $T_1= \left\lceil 2{\log_{\frac{3}{2}} (g/\epsilon)}\right\rceil$. 

\For{$t\leftarrow  1 $ to $T_1$}

\State Initialize  $L=%\max\left\{
\frac{3g^{1-\alpha}}{C_2(1-\alpha)}$,  %,\sqrt{\frac{5dg}{C_3}}\right\}$,
$\mathcal{B}=[-L,L]^d $, $C=C_0=\frac{g}{L}$.
\State Let $r=\max\{g^{\frac{(d+4)-\alpha(d+3)}{d+5}}, \frac{5C_0}{C_2} \}$,  $T_2=d\left\lceil {\log_{\frac{5}{4}} (L/r)}\right\rceil^+$, $\Delta=\frac{C_0}{2T_2}$, $\delta_\textup{r}=\frac{\delta}{2T_1T_2}$. 

%Let %\in[\frac{5C_0}{C_3}, 3C_0]$
\While{$L\geq r$}%{$t_2\leftarrow  1 $ to $ T_2$}


\State  $(\mathcal{B}, \boldsymbol{x})$ =Reduce$(\mathcal{B}, \boldsymbol{x}, C, \Delta, \delta_{\textup{r}})$. 

\State Let $L$ be the longest edge length in $\mathcal{B}$, $C=C+2\Delta$. 

\EndWhile

\State $\boldsymbol{x}=$Uniform search$(\mathcal{B}, \boldsymbol{x}, \frac{g}{3}, \frac{\delta}{2T_1})$,  $g=(\frac{2}{3})^{\alpha} g$
 %other half)$
\EndFor

\Return $\boldsymbol{x}$
%\EndWhile

%\State Let $D_0=g^?$, $r=g^?$
%\State local ball search $3r$
\EndProcedure

\

\Procedure{Uniform search}{$\mathcal{B}$, $\boldsymbol{x}$, $\epsilon_{\textup{u}},  \delta_{\textup{u}}$}

\State Let $\mathcal{Y}$ be an $\sqrt{\epsilon_{\textup{u}}/C_2}$-net of $\mathcal{B}$
%\State Estimate $f(\boldsymbol{x})$ with $\tilde{\Theta}(g^{-2})$ samples, and let the result be $\hat{f}_{\boldsymbol{x}}$.
%\State Let $\mathcal{Y}$ be a finite subset in $\mathcal{B}$ being a $\sqrt{g/3\max\{C_3,1\}}$-covering with size $O(\textup{Vol}{(\mathcal{B})}/g^{d/2})$
%\State For each $y\in\mathcal{Y}$, estimate $f(y)$ with $\tilde{\Theta}(g^{-2}%\log a
%)$ samples, and let the result be $\hat{f}_{\boldsymbol{y}}$.
%\State Let $\mathcal{Y}^*=\{\boldsymbol{y}\in\mathcal{Y} \ |\ \hat{f}_{\boldsymbol{y}}<\hat{f}_{\boldsymbol{x}}- \frac{C}{2}||\boldsymbol{y}-\boldsymbol{x}||_2\}$ and 
%the minimizer within $\mathcal{Y}^*$ be $\boldsymbol{y}^*$.
%\State Let  $\boldsymbol{y}^*=\textup{argmin}_{\boldsymbol{y}\in\mathcal{Y}}\  \hat{f}_{\boldsymbol{y}}-\frac{1}{2}g\cdot \mathbbm{1}(\boldsymbol{y}=\boldsymbol{x})$
%\doWhile {$F_{\boldsymbol{y}^*}\leq \hat{f}_{\boldsymbol{x}}$}

\Return $\boldsymbol{y}^*=\textup{argmin}_{\boldsymbol{y}\in\mathcal{Y}\cup\{\boldsymbol{x}\}}$ Sample$\left(\boldsymbol{y},\frac{\epsilon_{\textup{u}}}{4},\frac{\delta_{\textup{u}}}{|\mathcal{Y}|+1} \right)-\frac{1}{2}\epsilon_{\textup{u}}\cdot \mathbbm{1}(\boldsymbol{y}=\boldsymbol{x})$
%\doWhile {$F_{\boldsymbol{y}^*}$

\EndProcedure
\end{algorithmic}
\end{algorithm}

Within each iteration of the outer loop, the algorithm first executes a global search using the Reduce function to locate a dominant point within a hypercuboid. Formally, recall that the Reduce function reduces the longest edge length of $\mathcal{B}$ by a factor of at least $\frac{4}{5}$. The inner loop halts within $T_2$ iterations. By Proposition \ref{prop:redu}, the end result of the inner loop is a dominant point of the returned set  $\mathcal{B}$ with parameter $C= 2C_0$ w.p. $1-\frac{\delta}{2T_1}$, if $\boldsymbol{x}$ is initially a dominant point of $[-L,L]^{d}$ with $C=C_0$. From proposition \ref{prop:ele}, this condition is satisfied if $f(\boldsymbol{x})-f^*\leq g$. 

%which 






A local search follows the inner loop to return a point that is close to the global minima. 
%We present the following guarantee for the local search steps.
\begin{prop}\label{prop:ukey}
Given any inputs $\mathcal{B}$, $\boldsymbol{x}$, the function Uniform Search returns a point $y^*$ satisfying the following conditions w.p. $1-\delta_{\textup{u}}$. If $\mathcal{B}$ contains a global minimum of $f$, we have  $f(\boldsymbol{y}^*)-f^*\leq 2\epsilon_{\textup{u}}$; otherwise, we have $f(\boldsymbol{y}^*)-f(\boldsymbol{x})\leq 0$.
\end{prop}

Combining Proposition \ref{prop:dom_key} and Proposition \ref{prop:ukey}, the point $\boldsymbol{x}$ returned from the Uniform Search satisfies $f(\boldsymbol{x})-f^*\leq g$ for the updated $g$, w.p. $1-\frac{\delta}{2T_1}$. Therefore, by induction, we always have $f(\boldsymbol{x})-f^*\leq g$ at the beginning of each outer-loop iteration, and the initial condition is provided by the boundedness of $f$. After $T_1$ iterations, we have $f(\boldsymbol{x})-f^*\leq \left(\frac{2}{3}\right)^{\alpha T_1}\left(\frac{4C_2}{C_1^2} \right)^{\frac{1}{2\alpha-1}} \leq \epsilon$, and the overall error probability from the union bound is at most $\delta$.  


%each inner finds $2c_0$ dominant point . Proposition \ref{prop:dom_key} either has min or same point has $(2/3)^{\alpha}$
~

The overall sample complexity can be bounded by counting the costs from the Reduce and Uniform Search functions. Within each outer loop, the sample complexity of each call of the Reduce function almost exponentially depends on the number of inner-loop iterations. Hence the total cost from the reduce function for each outer-loop iteration is $\tilde{O}\left(\frac{r^{\frac{d-5}{2}}}{\Delta^{\frac{d+3}{2}}}\log(\frac{r}{\Delta\delta_{\textup{r}}})\right)$ %todo: verify 
 for $d\leq 5$.\footnote{Here we presented a straightforward version of the search algorithm for readability. The polylog factor can be improved by letting $\Delta$ to be a function of $L$, which brings in exponential dependency on the number of inner loop iterations. Similar improvements can also be achieved by modifying the uniform search. } On the other hand, each uniform search costs $\tilde{O}\left(\frac{r^d}{g^{\frac{d+4}{2}}}\log\left(\frac{2T_1}{\delta}\right) \right)$. Both can be written as $\tilde{O}(g^{-2-d\frac{(d+3)(\alpha-1/2)}{d+5}}\log\left(\frac{2T_1}{\delta}\right))$. As a consequence, the overall sample complexity is given by $\tilde{O}{(\epsilon^{-2-d\frac{(d+3)(\alpha-1/2)}{d+5}})}$.

%\begin{remark}
%The lengths of the search steps for each KL aggregate is exponentially decaying. Therefore, it suffices to assume the conditions of $\mathcal{F}$ holds within a $O(1)$-radius hypersphere. 
%\end{remark}

%\subsection{pl theorm}

%remark: compared to 1d case, the inner loop gets closer. 

%\section{$d=6$}


==> app_pp5.tex <==
\section{Proof of Proposition \ref{prop:redu}}\label{app:pp5}
\begin{proof}
Let $\hat{f}(\boldsymbol{y})$ denote the value returned for each call of the Sample function.   By union bound and Proposition \ref{prop:sample}, we have $\hat{f}(\boldsymbol{y})\in [{f}(\boldsymbol{y})-\epsilon_{\textup{r}},{f}(\boldsymbol{y})+\epsilon_{\textup{r}}]$  for all sampled $\boldsymbol{y}$ w.p. $1-\delta_{\textup{r}}$. We will focus on this event in the rest of the proof. 


Depending on the value of $\boldsymbol{y}^*$, we consider two possible cases. First, if $\boldsymbol{y}^*=\boldsymbol{x}$, we 
%First, we consider the function 
let $F(\boldsymbol{y})\triangleq (C_0+2\Delta)||\boldsymbol{y}-\boldsymbol{y^*}||_2+f(\boldsymbol{y})$ and $\boldsymbol{y}_F\triangleq \textup{argmin}_{\boldsymbol{y}\in \mathcal{S}_p\cup\mathcal{S}_q}F(\boldsymbol{y}).$  %We prove that 
To prove that $\boldsymbol{y}^*$ is a dominant point on the new set, it suffices to show that $F(\boldsymbol{y}_F)>F(\boldsymbol{x})$. 
We prove this statement by contradiction. Assume that $F(\boldsymbol{y}_F)\leq F(\boldsymbol{x})$. 
By the dominant condition of $\boldsymbol{x}$ on $\mathcal{B}$, the point $\boldsymbol{y}_F$ can not be on the boundary of $\boldsymbol{B}$. 
Hence, we have $\nabla F(\boldsymbol{y}_F)$ is orthogonal to $\mathcal{S}_p$ and $\mathcal{S}_q$. 
 Therefore, the value of $F(\boldsymbol{y}_F)$ can be bounded by the sampled results using the smoothness condition.   

Without loss of generality, assume $\boldsymbol{y}_F\in \mathcal{S}_p$. We rely on the following fact to show a smoothness condition of $F$.
\begin{prop}\label{prop:balance}
For any real numbers $a<x<b$, both the outputs $p$, $q$ from Balanced Partition$(a,b,x)$ belong to $(a,b)$ and the distance from any of them to any other $4$ points belongs to % distance each of them is at least 
$[(b-a)/5, 4(b-a)/5]$. % away from any other $4$ points.
\end{prop}
%By elementary calculus, 
The above proposition provides a lower bound of $||\boldsymbol{y}-\boldsymbol{x}||_2$ for any $\boldsymbol{y}\in\mathcal{S}_{p}$. Hence, by taking the derivatives, one can show that 
\begin{align*}F(\boldsymbol{y})-F(\boldsymbol{y}_F)\leq\left(\frac{5(C_0+2\Delta)}{2(b_k-a_k)}+C_2\right)||\boldsymbol{y}_F-\boldsymbol{y}||_2^2\leq 2C_2||\boldsymbol{y}_F-\boldsymbol{y}||_2^2.
\end{align*}
We remind the reader the definition of $\epsilon$-net.
\begin{defn}[$\epsilon$-net]
Let $\mathcal{Y}$ be a subset of $\mathcal{S}$ and $\epsilon>0$ be a general parameter. We say $\mathcal{Y}$ is an $\epsilon$-\emph{net} of $\mathcal{S}$, if the packing radius of $\mathcal{Y}$ is no smaller than ${\epsilon}/2$, and the covering radius is no greater than $\epsilon$.
\end{defn}
By the covering property, there is a sampled point $\hat{\boldsymbol{y}}_F$ on $\mathcal{S}_p$ with  $||\boldsymbol{y}_F-\boldsymbol{y}||_2\leq \sqrt{\epsilon_\textup{r}/C_2}$. Consequently, 
\begin{align*}
    F(\hat{\boldsymbol{y}}_F)-F(\boldsymbol{y}_F)< 2\epsilon_{\textup{r}}.
\end{align*}
Recall that $f(\hat{\boldsymbol{y}}_F)$ is sampled with an error of at most $\epsilon_{\textup{r}}$. We have 
\begin{align*}
\hat{f}(\hat{\boldsymbol{y}}_F)+(C_0+2\Delta)||\boldsymbol{x}-\hat{\boldsymbol{y}}_F||_2-F(\boldsymbol{y}_F)< 3\epsilon_{\textup{r}}.
\end{align*}
Now we use the fact that
$\boldsymbol{y}^*=\boldsymbol{x}$ and $f(\boldsymbol{x})$ is also sampled with an accuracy of $\epsilon_{\textup{r}}$. % and the definition of $\boldsymbol{y}_F$.
\begin{align*}
    \hat{f}(\hat{\boldsymbol{y}}_F)+(C_0+\Delta)||\boldsymbol{x}-\hat{\boldsymbol{y}}_F||_2&\geq  \hat{f}(\hat{\boldsymbol{x}})> F(\boldsymbol{x})-\epsilon_{\textup{r}}. %\\
    %F({\boldsymbol{y}}_F)&\leq F(\hat{\boldsymbol{x}})
\end{align*}
Combine the above two inequalities, we have $F(\boldsymbol{y}_F)-F(\boldsymbol{x})> \Delta||\boldsymbol{x}-\hat{\boldsymbol{y}}_F||_2-4\epsilon_{\textup{r}}\geq 0$
from Proposition \ref{prop:balance}, which contradicts the assumption on $\boldsymbol{y}_F$. %Hence, $\boldsymbol{y}_F\notin \mathcal{S}_p$. By symmetry, $\boldsymbol{y}_F\notin \mathcal{S}_q$ as well. Then we can conclude that $\boldsymbol{y}_F=\boldsymbol{x}$.

~


For the other case, we have $\boldsymbol{y}^*\in \mathcal{S}_p\cup \mathcal{S}_q$. 
Then by the sampling guarantee and the definition of $\boldsymbol{y}^*$, we have 
\begin{align*}
f(\boldsymbol{x})-f(\boldsymbol{y}^*)\geq \hat{f}(\boldsymbol{x})-\hat{f}(\boldsymbol{y}^*)-2\epsilon_{\textup{r}}\geq (C_0+\Delta)||\boldsymbol{x}-\boldsymbol{y}^*||_2 -2\epsilon_{\textup{r}}. 
\end{align*}

Recall that $\Delta||\boldsymbol{x}-\boldsymbol{y}^*||\geq 2\epsilon_{\textup{r}}$ can be implied from Proposition \ref{prop:balance}. The above inequality shows that 
\begin{align*}
f(\boldsymbol{x})-f(\boldsymbol{y}^*)\geq C_0||\boldsymbol{x}-\boldsymbol{y}^*||_2.
\end{align*}

Using triangle inequality, $\boldsymbol{y}^*$ is also a dominant point of $\mathcal{B}$ with $C=C_0$. 
Obviously, the same holds for a larger parameter $C=C_0+2\Delta$.


Now without loss of generality, we can assume that  $\boldsymbol{y}^*\in \mathcal{S}_p$. It remains to show that 
$F(\boldsymbol{y})> F(\boldsymbol{y}^*)$ for any $\boldsymbol{y}\in\mathcal{S}_q$. Similar to the first case, we assume the opposite and define $\boldsymbol{y}_q\triangleq \textup{argmin}_{\boldsymbol{y}\in\mathcal{S}_q}F(\boldsymbol{y})$. Recall that $\boldsymbol{y}^*$ dominates $\boldsymbol{B}$. The point $\boldsymbol{y}_q$ is not on the boundary of $\boldsymbol{B}$.  Following the same arguments used in the first case, one can show the existence of $\hat{\boldsymbol{y}}_F\in\mathcal{S}_{\textup{net},q}$ for the following inequalities to hold. 
\begin{align*}
    \hat{f}(\hat{\boldsymbol{y}}_F)+(C_0+2\Delta)||\boldsymbol{y}^*-\hat{\boldsymbol{y}}_F||_2&-F(\boldsymbol{y}_F)< 3\epsilon_{\textup{r}}\\
      \hat{f}(\hat{\boldsymbol{y}}_F)+(C_0+\Delta)||\boldsymbol{x}-\hat{\boldsymbol{y}}_F||_2> F(\boldsymbol{y^*})&+(C_0+\Delta)||\boldsymbol{x}-\hat{\boldsymbol{y}^*}||_2-\epsilon_{\textup{r}}.
\end{align*}
Combine the above inequalities and use the triangle inequality, we can conclude that 
\begin{align*}
F(\boldsymbol{y}_F)-F(\boldsymbol{y^*})>\Delta||\boldsymbol{y}^*-\hat{\boldsymbol{y}}_F||_2-4\epsilon_{\textup{r}}\geq 0.
\end{align*}
~

Finally, we prove the sample complexity.  
We use the following well know upper bound for the size of $\epsilon$-nets. 
\begin{prop}
For any fixed $d$ and any set $\mathcal{B}$ that belongs to $\mathbb{R}^d$, an $\epsilon$-net of $\mathcal{B}$ exists. If
\begin{align*}
V\triangleq \textup{Vol}\{\boldsymbol{x}\in\mathbb{R}^d\ |\  \exists\ \boldsymbol{y}\in \mathcal{B},  ||\boldsymbol{x}-\boldsymbol{y}||_2\leq {\epsilon}/{2}\}
\end{align*}
is finite, then any $\epsilon$-net is finite, with a size of $O(V/\epsilon^d)$.
\end{prop}
The algorithm runs $O(|\mathcal{S}|)$ numbers of Sample calls. Given the stated assumptions and the above proposition, we have 
\begin{align*}
|\mathcal{S}|=O\left(\frac{\prod_{j\neq k}(b_j-a_j+\epsilon_{\textup{r}})}{\epsilon_{\textup{r}}^{d-1}}\right)=O\left(\frac{(b_k-a_k)^{\frac{d-1}{2}}}{{\Delta}^{\frac{d-1}{2}}}\right).
\end{align*}
Hence, the overall sample complexity is $O\left(\frac{|\mathcal{S}|}{\epsilon_{\textup{r}}^2}\log (\frac{|\mathcal{S}|}{\delta})\right)={O}\left(\frac{ (b_k-a_k)^{\frac{d-5}{2}}}{\Delta^{\frac{d+3}{2}}}\log(\frac{b_k-a_k}{\Delta\delta})\right).$ 
\end{proof}


==> appa.tex <==
The main intuition of gradient-based method is as follows. Starting from any point $\vct x\in\mathbb{R}$, if one can measure an approximated gradient of $f$ at the same point, %on a direction specified by a unit vector $\vct u$,
 then due to the smoothness condition, the function value for the updated point $\vct x'=\vct x- \frac{1}{2C_2} %\vct u\vct u \cdot
  \nabla f (\vct x) $ satisfies
%\begin{align*}
$f(\vct x')\leq f(\vct x)- \frac{1}{4C_2^2}||\nabla f (\vct x)||_2^2$.
%\end{align*} 
%todo: verify d dependency


More specifically, when using zero-th order measurements, one can measure the partial gradient $f_{\vct u} = \vct u \cdot \nabla f$ for any unit vector $\vct u$ and achieve a decent of $\frac{1}{4C_2^2}||\vct u \cdot \nabla f (\vct x)||_2^2$. In expectation, we have $\mathbb{E}[|f_{\vct u}|^2]=\frac{1}{d}||\nabla f (\vct x)||_2^2$ for uniformly random $\vct u$. Hence, we can measure $\min\{f_{\vct u}, 0\}$ up to an error of $O(\frac{1}{\sqrt{d}} ||\nabla f (\vct x)||_2)$ with high probability by sampling at $\vct x$ and $\vct x + \frac{z}{2C_2 \sqrt{d}}\vct u$ for any lower bound $z\in (0,  ||\nabla f (\vct x)||_2]$. It takes $O(\log \frac{1}{\delta})$ random samples of $\vct u$ to observe $f_{\vct u}\geq \frac{1}{\sqrt{d}} ||\nabla f (\vct x)||_2$ with probability $1-\delta$, and the sample complexity for each fixed $\vct u$ is $\tilde{O}(\frac{d^2}{z^4} \log \frac{1}{\delta})$. 


Recall the KL condition. It takes $O(dg^{1-2\alpha})$ such decent steps to reduce $f(\vct x)-f^*$ by half when $f(\vct x)-f^* \leq g$, and it is achieved by choosing $z=\Theta(g^{\alpha})$. Hence, the overall sample complexity is $\tilde{O}(d^3\epsilon ^{1-6\alpha}\log^2 \frac{1}{\delta})$ to achieve a simple regret $\epsilon$ with error probability $\delta$. This implies a complexity upper bound of $O(d^3\epsilon ^{1-6\alpha})$ for achieving an expected simple regret of $\epsilon$.


%Note that it takes 
%Hence, one can 
%one can achieve a descent of $\m$

%f $|f_{\vct u}|$ is lower bounded by $x$



 %up to error $z$ by sampling at $\vct x$ and $\vct x+z \vct u$.  

For clarity, we state a simplified procedure in Algorithm \ref{algA}, which achieves the same $\tilde{O}(d^3\epsilon ^{1-6\alpha}\log^2 \frac{1}{\delta})$ complexity guarantee. %approx, fz>f/4/sqrt d w.p.0.1

\begin{algorithm}
\caption{Gradient-Based Method}\label{algA}
\begin{algorithmic}
%\Procedure{SGD}{$\epsilon$, $\delta$} %, $\Delta$}
%\State Let $\boldsymbol{y}^*=\boldsymbol{x}_0$
\State Initialize $\boldsymbol{x}=\boldsymbol{0}$, $g=\left(\frac{4C_2}{C_1^2} \right)^{\frac{1}{2\alpha-1}}$.
%\While {$g\geq \epsilon$} 
 Let $T_1= \left\lceil 2{\log_{\frac{3}{2}} (g/\epsilon)}\right\rceil$. 

\For{$t_1\leftarrow  1 $ to $T_1$}

%\State Initialize  $L=%\max\left\{
%\frac{3g^{1-\alpha}}{C_2(1-\alpha)}$,  %,\sqrt{\frac{5dg}{C_3}}\right\}$,
%$\mathcal{B}=[-L,L]^d $, $C=C_0=\frac{g}{L}$.
\State Let $z=C_1 (\frac{2}{3}g)^\alpha$,  $r=\frac{z}{8C_2\sqrt{d}}$, $\delta_t=\frac{\delta}{2\cdot 2^{T_1-t}}$, $T_2=\left\lceil {\frac{4g}{3C_2 r^2}}\right\rceil \cdot \left\lceil {\log_{\frac{10}{9}} (\frac{1}{\delta})}\right\rceil^+$. 

%Let %\in[\frac{5C_0}{C_3}, 3C_0]$

\For{$t_2\leftarrow  1 $ to $T_2$}

\State Let $\vct u$ be uniformly random from the unit hypersphere 

\State Let $D={\textup{Sample}\left(\boldsymbol{x},\frac{C_2r^2}{4},\frac{\delta_{t}}{4T_2} \right)}-{\textup{Sample}\left(\boldsymbol{x}+r\vct u,\frac{C_2r^2}{4},\frac{\delta_{t}}{4T_2} \right)}$

\If {$D\geq \frac{C_2r^2}{2}$}

\State $\vct x=\boldsymbol{x}+r\vct u$

\EndIf
\EndFor

\State  $g=(\frac{2}{3})^{\alpha} g$
 %other half)$
\EndFor

\Return $\boldsymbol{x}$
%\EndWhile

%\State Let $D_0=g^?$, $r=g^?$
%\State local ball search $3r$
%\EndProcedure

%\Return $\boldsymbol{y}^*=\textup{argmin}_{\boldsymbol{y}\in\mathcal{Y}\cup\{\boldsymbol{x}\}}$ Sample$\left(\boldsymbol{y},\frac{\epsilon_{\textup{u}}}{4},\frac{\delta_{\textup{u}}}{|\mathcal{Y}|+1} \right)-\frac{1}{2}\epsilon_{\textup{u}}\cdot \mathbbm{1}(\boldsymbol{y}=\boldsymbol{x})$
%\doWhile {$F_{\boldsymbol{y}^*}$

\end{algorithmic}
\end{algorithm}

==> appkl_1dd.tex <==
\section{Proof details on inequality \eqref{ineq:1ds2}}\label{app:pkl1dd}


Here we used the fact that $L$ is reduced by a factor of  $\frac{1}{2}$  within each global search step. Therefore, we always have $2L\geq L_{\textup{th}}$ within the loop, and then inequality (\ref{ineq:1ds2}) implies that $ f(x_{\textup{c}}\pm L)\geq  f(x_{\textup{c}})-2C_0\cdot L.$

For the induction proof, we first check the initial condition. When $L=L_0$, 
\begin{align*}f(x_{\textup{c}}\pm L)\geq f^*\geq f(x_{\textup{c}})-g_t=f(x_{\textup{c}})-C_0L_0\geq f(x_{\textup{c}})-\left(C_0+\Delta_C\right) L.
\end{align*}
Hence, inequality \eqref{ineq:1ds2} holds at the beginning of the global search, %which is implied by  $f(x_{\textup{c}})-f^*\leq g_{t}=C_0L_0$ and $ f(x_{\textup{c}}\pm L)\geq f^*$. Hence,  
and it suffices to consider the case where $L_0$ is large enough to enter the global search loop.  


Then assume inequality \eqref{ineq:1ds2} holds at the beginning of any given search step, we prove that it holds at the end of the same step. There are three possible cases. When $x_{\textup{c}}$ is not updated, the interval is updated to $[x_{\textup{c}}-\frac{L}{2},x_{\textup{c}}+\frac{L}{2}]$. From Proposition \ref{prop:sample} and the argmin condition, we have the following bounds with high probability,
\begin{align*}f\left(x_{\textup{c}}\pm\frac{L}{2}\right)\geq f(x_{\textup{c}})-\left(C_0+\Delta_C\right)\cdot\frac{L}{2}-2\epsilon_{L}> f(x_{\textup{c}})-\left(C_0+2^{\frac{2}{3}}\Delta_C\right)\cdot\frac{L}{2},
\end{align*}
 which proves the induction statement. Among the other two cases, without loss of generality, we assume %$f_1\geq f_2$ without loss of generality, and
 the updated interval is given by $[x_{\textup{c}},x_{\textup{c}}+L]$ in terms of the initial parameters. %Note that $\Delta_C\leq C_0$? before $L$ is updated.
 From Proposition \ref{prop:sample} and the induction assumption, we have 
\begin{align*}
    f\left(x_{\textup{c}}+\frac{L}{2}\right)%-f\left(x_{\textup{c}}+L\right)
    &\leq f(x_{\textup{c}})%-f(x_{\textup{c}}+L)
    -\left(C_0+\Delta_C\right)\cdot\frac{L}{2}+2\epsilon_{L}\\
    &\leq f(x_{\textup{c}}+L)+\left(C_0+\Delta_C\right)\cdot\frac{L}{2}+2\epsilon_{L} \\
    &< f(x_{\textup{c}}+L)+(C_0+2^{\frac{2}{3}}\Delta_C)\cdot \frac{1}{2}L.
\end{align*}
We also have
\begin{align*}
    f\left(x_{\textup{c}}+\frac{L}{2}\right)\leq f\left(x_{\textup{c}}\right)<f\left(x_{\textup{c}}\right) +(C_0+2^{\frac{2}{3}}\Delta_C)\cdot \frac{1}{2}L. 
\end{align*}
Therefore, the induction statement for the updated interval also holds in these case and the proof for global search phase is concluded.

%at %the beginning and
%the end of each search step. 




%from the smoothness of $f$ and KL inequality, one can ensure that a global minima exists within the initialized interval. Formally, we have the following proposition for any $d$, 


% can be performed . %to estimate the $f$ values within. 






%We show that after each iteration of the global search, the minimum of $f$ within the interval approximates $f^*$ with high probability. The approximation requirement is that  %we prove that 

%We prove this inequality by induction: % over the number of iterations. 
%consider any fixed iteration and assume that inequality \ref{ineq:1din} holds at the beginning, we aim to show that it is maintained at the end.  %at least one global minima of $f$ belongs to $[x_{\textup{c}}-L,x_{\textup{c}}+L]$ at the beginning of the iteration, we prove that this property is maintained at the end. 
%Note that the updated interval always includes $\left[x_\textup{c}-\frac{L}{3},x_\textup{c}+\frac{L}{3}\right]$, it suffices to consider the case where this interval contains no good approximation of global minima of $f$, i.e.,  $f\left(x\right)-f^*> \frac{\epsilon}{4}$ for any $x\in \left[x_\textup{c}-\frac{L}{3},x_\textup{c}+\frac{L}{3}\right]$. 

%Recall that $f(0)\geq f(x_{\textup{c}})$. The KL inequality implies that the differential $f'(x_{\textup{c}})$ is non-zero. Without loss of generality, we assume it is positive. Then $f$ needs to be increasing on $\left[x_\textup{c}-\frac{L}{3},x_\textup{c}\right]$ and $f(x_\textup{c}-\frac{L}{3})\leq f(x_\textup{c})-\frac{L}{3}\cdot C_1(\frac{\epsilon}{4})^\alpha$. Specifically, the positivity of $f'(x_{\textup{c}})$ ensures that $f$ is increasing in a neighbourhood $[y,x_\textup{c}]$ for some $y<x_\textup{c}$. Let $y^*$ be the infimum of all such $y$ in $\left[x_\textup{c}-\frac{L}{3},x_\textup{c}\right]$. We aim to prove that $y^*=x_\textup{c}-\frac{L}{3}$. By definition, we have $f(y)\leq f(x)\leq f(0)$ for all $y\in (y^*,x_\textup{c}]$. Hence, differentiability holds for all such $y$ and $f'(y)\geq 0$. Taking the limit of the smoothness condition, 
%we have $f(y^*)\leq \lim_{x\rightarrow y^{*-}} f(x)$. Therefore, the monotonicity of $f$ extends to the boundary $y^*$ and  $f'(y^*)\geq 0$ as well. From the KL inequality, $f'(y^*)$ is strictly positive. Thus, $y^*$ has to be on the boundary $x_\textup{c}-\frac{L}{3}$ to be consistent with its definition. Then, one can obtain an explicit upper bound of $f(x_\textup{c}-\frac{L}{3})$ by the mean value theorem.


%smoothness condition can be applied at $y^*$, and 
%is right-continuous .  

%Then $y^*$ has to be a local minima of $f$ on domain $\left[x_\textup{c}-\frac{L}{3},x_\textup{c}\right]$  is increasing in $[y^*,x_\textup{c}]$. 


%Assume the contrary and let $y$ be the infimum on $\left[x_\textup{c}-\frac{L}{3},x_\textup{c}\right]$ that $[y,x_{\textup{c}}]\subseteq \mathcal{X}$. 


%Using the smoothness condition, the function $\overline{f}(x)\triangleq\min\{f(x),f(0)\}$ is quasi-concave on $\left[x_\textup{c}-\frac{L}{3},x_\textup{c}+\frac{L}{3}\right]$, otherwise .


%is continuous on 





%Note that Proposition \ref{prop:sample} guarantees that both $f\left(x_\textup{c}-\frac{L}{3}\right)$ and $f\left(x_\textup{c}+\frac{L}{3}\right)$ are estimated up to an error of $\frac{1}{3}L\cdot  C_2 \left(\frac{\epsilon}{4}\right)^{\alpha}$, each with an error probability of $\frac{\delta}{6L}\epsilon^{\frac{5-4\alpha}{6}}$. Therefore, we have $$f_1-f_2\geq f\left(x_\textup{c}-\frac{L}{3}\right)-f\left(x_\textup{c}+\frac{L}{3}\right) - \frac{2}{3}L\cdot  C_2 \left(\frac{\epsilon}{4}\right)^{\alpha}>0$$ w.p. $1-\frac{\delta}{3L}\epsilon^{\frac{5-4c}{6}}$. 
%When the above inequality is true, by monotonicity of $f$, the new interval contains the minimum of $f$ within $[x_\textup{c}-L,x_\textup{c}+L]$. Then by the induction assumption, we also have inequality (\ref{ineq:1din}) for the new interval. Recall that $L$ decays exponentially. One can apply the union bound %for the overall process
%to show that the overall error probability for violating inequality (\ref{ineq:1din}) %for the global search phase
%is at most $\frac{1}{2}\delta$. %Hence, 

~


==> checklist.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

\iffalse
%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%
\fi

\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
 \answerYes{}
  \item Did you describe the limitations of your work?
 \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
 \answerNA{This is a theoretical work and it doesn't apply. }
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
 \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
     \answerYes{}
          \item Did you include complete proofs of all theoretical results?
    \ \answerYes{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
 \answerNA{}
   \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
 \answerNA{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
\answerNA{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
\answerNA{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
\answerNA{}
  \item Did you mention the license of the assets?
\answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
\answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
\answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
\answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
\answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
\answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
\answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

